A Review on Recommendation Systems: Context-aware to Social-based

The number of Internet users had grown rapidly enticing companies and cooperations to make full use of recommendation infrastructures. Consequently, online advertisement companies emerged to aid us in the presence of numerous items and users. Even as a user, you may find yourself drowned in a set of items that you think you might need, but you are not sure if you should try them. Those items could be online services, products, places or even a person for a friendship. Therefore, we need recommender systems that pave the way and help us making good decisions. This paper provides a review on traditional recommendation systems, recommendation system evaluations and metrics, context-aware recommendation systems, and social-based recommendation systems. While it is hard to include all the information in a brief review paper, we try to have an introductory review over the essentials of recommendation systems. More detailed information on each chapter will be found in the corresponding references. For the purpose of explaining the concept in a different way, we provided slides available on https://www.slideshare.net/MahdiSeyednejad/recommender-systems-97094937.

==> 5_modern/5_modern.tex <==
\chapter{Modern Topics in Recommender Systems}
\label{ch:modern}
In this section, we briefly introduce a number of modern topics in the recommender system studies. For more details, a set of research and survey papers are provided as a reference to guide the reader to appropriate articles. The following topics are among ongoing studies that can be 

\section{Research Paper Recommender System}
One of the major applications of the recommender systems is to recommend a set of relevant and useful papers to a scholar in the right time.
%
In addition to the time limitations, the issue of copyright prevent a recommender system to access to the full content of a paper. 
%
Two popular approaches are context-based collaborative filtering~\cite{liu2015context} and co-citation~\cite{mcnee2002recommending}. In the former, the authors use the network of citations to create the rating matrix. The latter takes into account the assumption that if two paper cite same papers, they are similar. 
%

Haruna et al.~\cite{haruna2017collaborative} propose a collaborative method that uses the public data about the paper for the recommendation purposes. In their method, if author {\it A} writes a paper {\it P}, they consider recommending papers that have two conditions: They are co-cited with the paper {\it P} of the author {\it A}, and have common references with paper {\it P}. They show their method outperforms context-based collaborative filtering and co-citation techniques. Another method for research paper recommendation is to analyze the topics of the papers. Pan et al.~\cite{pan2010research} 

User interests can give a hint towards finding related papers. Sugiyama et al.~\cite{sugiyama2010scholarly} ...


\section{Recommender Systems Based on Bio-inspired Algorithms}


\section{Recommender Systems for Education}

\section{More topics on Recommender Systems}

==> app_emoji/5_emoji.tex <==
\appendix
\newcommand{\light}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/light}}
\newcommand{\medLight}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/light_medium}}
\newcommand{\medium}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/medium}}
\newcommand{\medDark}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/dark_medium}}
\newcommand{\dark}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/dark}}

\newcommand{\joy}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/face_with_tears_of_joy}}
\newcommand{\smiling}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/smiling_face}}
\newcommand{\grinningFace}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/grinning_face}}


\newcommand{\monkey}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/monkey_face}}
\newcommand{\fox}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/fox_face}}
\newcommand{\cactus}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/cactus}}

\newcommand{\grape}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/grapes}}
\newcommand{\wine}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/wine_glass}}
\newcommand{\fries}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/french_fries}}

\newcommand{\globe}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/globe_showing_Americas}}
\newcommand{\plane}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/airplane}}
\newcommand{\train}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/locomotive}}

\newcommand{\wrestle}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/women_wrestling}}
\newcommand{\biking}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/person_biking}}
\newcommand{\ball}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/soccer_ball}}

\newcommand{\camera}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/movie_camera}}
\newcommand{\phone}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/telephone}}
\newcommand{\battery}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/battery}}

\newcommand{\entry}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/no_entry}}
\newcommand{\water}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/potable_water}}
\newcommand{\rept}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/repeat_button}}

\newcommand{\iran}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/iran}}
\newcommand{\brazil}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/brazil}}
\newcommand{\usa}{\includegraphics[height=1.5\fontcharht\font`\B] {figEmoji/usa}}


\renewcommand\chaptername{Appendix}
\chapter{Appendix - Emoji}
\label{ch:emoji}

\section{Unicode}
In 1968, the American Standard Code for Information Interchange (ASCII) was standardized. ASCII defined numeric codes for various characters, with the numeric values running from 0 to 127, but it was limited to English letters. For example, there was an ‘e’, but no ‘é’ or ‘Í’.  Even if you changed coding  to another language, you could not use different language letters at the same time. Ultimately, languages which required accented characters couldn’t be faithfully represented in ASCII\footnote{https://docs.python.org/2/howto/unicode.html}. 

The Unicode standard describes how characters are represented by code points. A character is represented on a screen or on paper by a set of graphical elements that are called glyphs. For example {\bf A} has three glyphs: ``{\bf /}” and ``{\bf -}" and ``{\bf \textbackslash}". A Unicode string is a sequence of code points, which are numbers from ``0" to ``0x10FFFF". This sequence needs to be represented as a set of bytes (meaning, values from 0–255) in memory. The rules for translating a Unicode string into a sequence of bytes are called an encoding. There are some important notations used in Unicode terminology as following\footnote{https://techterms.com/definition/characterencoding}:
\begin{itemize}
\item {\bf code unit} --- A code unit is the unit of storage of a piece of an encoded code point. In UTF-8 this means 8-bits, in UTF-16 this means 16-bits. A single code unit may represent a full code point, or part of a code point. 
\item {\bf Code point} --- A code point is the atomic unit of information. Text is a sequence of code points. Each code point is a number which is given meaning by the Unicode standard. 
In character encoding terminology, a code point or code position is any of the numerical values that make up the code space. Unicode comprises 1,114,112 code points in the range $0_{hex}$ to $10FFFF_{hex}$. The Unicode code space is divided into seventeen planes (the basic multilingual plane, and 16 supplementary planes), each with 65,536 (= 216) code points. The total size of the Unicode code space is 17 x 65,536 = 1,114,112.

\end{itemize}

\section{Emoji}
Pictures are worth a thousand words. Using pictures was an ancient way to convey an idea. Pictures are somehow independent of languages. They can modify the true feelings behind the text. These days, with the tremendous growth of Internet users, people tend to send or post short messages, but, sometimes, the true feeling behind the text is lost. That is why several pictures has been introduced to express the feeling better and somehow complete the text. Nowadays, we know those pictures as emoji.

Emoji are pictographs (pictorial symbols) that are typically presented in a colorful cartoon form and are used inline in text. Emoji represent things such as faces, weather, vehicles and buildings, food and drink, animals and plants, or icons that represent emotions, feelings, or activities. Emoji were initially used by Japanese mobile operators. The first emoji was created in 1998 in Japan by Shigetaka Kurita, who was part of the team working on NTT DoCoMo's i-mode mobile Internet platform. The word emoji comes from the Japanese \footnote{http://unicode.org/reports/tr51/index.html}:

\section{Emoji Sequences}
In Unicode technical report \#51, the Unicode organization defines different sequences of Unicodes that can generate emoji:\\
\begin{minipage}{15cm}
  \texttt{emoji\_flag\_sequence :=  regional\_indicator regional\_indicator}\\
\texttt{emoji\_combining\_sequence := (emoji\_character | emoji\_presentation\_sequence | text\_presentation\_sequence) non\_spacing\_mark\textsuperscript{$\ast$}   }\\
\texttt{emoji\_core\_sequence  :=   emoji\_combining\_sequence | emoji\_modifier\_sequence | emoji\_flag\_sequence}\\
\texttt{emoji\_zwj\_element :=  emoji\_character | emoji\_presentation\_sequence | emoji\_modifier\_sequence}\\
\texttt{emoji\_zwj\_sequence  :=   emoji\_zwj\_element ( ZWJ emoji\_zwj\_element)\textsuperscript{+}}\\
\texttt{emoji\_sequence :=  emoji\_core\_sequence | emoji\_zwj\_sequence}\\
\end{minipage}

We have tried to create a tree that represents the way that an emoji can be extracted from emoji sequences. Figure~\ref{fig:emojiTree} shows that tree along with three special codes that represent zero width joiner and the style of emoji.

\begin{figure}[ht]
\centering
\includegraphics[trim={0cm 0cm 0cm 0},clip, width=0.8\textwidth]{figures/emoji_tree}
\caption{Tree of emoji generating based on emoji sequences.}
\label{fig:emojiTree}
\end{figure}

Figure~\ref{fig:emoji_example} shows how a typical emoji is produced by a sequence of codes. In this example, the special character ZWJ (Zero Width Joiner) is used to join two concepts. The last part of the code implies that this should be displayed by emoji style, not text style.

\begin{figure}[ht]
\centering
\includegraphics[trim={1cm 1cm 1cm 1cm},clip, width=0.85\textwidth]{figures/emoji_code_example}
\caption{An example of generating an emoji code}
\label{fig:emoji_example}
\end{figure}

\section{Emoji Modifier and Codes}
Five symbol modifier characters were added with Unicode 8.0 to provide a range of skin tones for human emoji\footnote{https://en.wikipedia.org/wiki/Emoji}. Table~\ref{tab:emoji_skin} shows the codes and description related to these skin tones.

\begin{table}[ht]
\caption{Unicode and description for skin tone as modifier for emoji}
\begin{center}
  \resizebox{0.8\textwidth}{!}{%
  	\tabcolsep=0.2cm
    \begin{tabular}{l l l c}
     \toprule
      Code & Description & Name& Sample \\
       \midrule
       U+1F3B & light skin tone  & EMOJI MODIFIER FITZPATRICK TYPE-1-2 & \light  \\
       U+1F3C & medium-light skin tone  & EMOJI MODIFIER FITZPATRICK TYPE-3 & \medLight   \\
       U+1F3D & medium skin tone  & EMOJI MODIFIER FITZPATRICK TYPE-4 & \medium  \\
       U+1F3E & medium-dark skin tone  & EMOJI MODIFIER FITZPATRICK TYPE-5 & \medDark   \\
       U+1F3F & dark skin tone  & EMOJI MODIFIER FITZPATRICK TYPE-6 & \dark   \\
      \bottomrule
    \end{tabular}%
    }
\end{center}
\label{tab:emoji_skin}
\end{table}

% \begin{figure}[ht]
% \centering
% \includegraphics[trim={1cm 1cm 1cm 1cm},clip, width=0.85\textwidth]{figures/emj_skin}
% \caption{Unicode and description for skin tone as modifier for emoji.}
% \label{fig:emoji_skin}
% \end{figure}

Furthermore, table~\ref{tab:emoji_number} shows more details about emoji with the number of each category. For example, the number of ``Emoji_Combining_Sequence: Keycaps'' is 12 and the subtotal to that row of the table is 1100 (1011+12). The emoji have been categorized by their meaning or the field of use. Table~\ref{tab:emoji_order} shows this ordering with some samples from each group. IT should be noted that each order has some sub-orders. For example,  ``Smiley \& People'' category has sub-orders such as {\it Face-positive}, {\it Face-neutral}, {\it Face-negative}, {\it Face-sick}, etc.


\begin{table}[ht]
\caption{Counting emoji based on their Unicode and sequence}
\begin{center}
  \resizebox{0.85\textwidth}{!}{%
  	\tabcolsep=0.2cm
    \begin{tabular}{l l c}
     \toprule
      Type & Count & Subtotal\\
       \midrule
       Singletons & 1126 & 1126 \\
       Incomplete Singletons: 12 keycap base characters, 26 RI characters & -38 & 1088   \\
       Emoji Combining Sequence: Keycaps & 12 & 1100  \\
       Emoji Flag Sequence: Valid RI sequences & 258 & 1358 \\
       Emoji Modifier Sequence: Skin tones & 430 & 1788  \\
       Emoji ZWJ Sequence: Gendered Role, with object & 192 & 2011  \\
       Emoji ZWJ Sequence: Gendered Role, with sign & 72 & 2083 \\
       Emoji ZWJ Sequence: Gendered Activity, with sign & 196 & 2279 \\
       Emoji ZWJ Sequence: Gendered Gestures, with sign & 108 & 2387 \\
       Emoji ZWJ Sequence: Other & 2 & 2389 \\
	   Typically duplicating ZWJ sequences & -191 & 2198 \\
      \bottomrule
    \end{tabular}%
    }
\end{center}
\label{tab:emoji_number}
\end{table}


% \begin{figure}[ht]
% \centering
% \includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=0.85\textwidth]{figures/emj_number}
% \caption{Counting emoji based on their Unicode and sequence}
% \label{fig:emoji_number}
% \end{figure}

\begin{table}[ht]
\caption{Major orders of emoji with samples and sub-orders}
\begin{center}
  \resizebox{0.8\textwidth}{!}{%
  	\tabcolsep=0.2cm
    \begin{tabular}{l c l}
     \toprule
      Major orders & Samples & Some sub-orders \\
       \midrule
       Smiley \& People & \smiling \thinspace \joy \thinspace \grinningFace & face-positive, face-neutral, face-negative \\
       Animals \& Nature & \monkey \thinspace \fox \thinspace \cactus & animal-mammals, animal-birds, plant-other  \\
       Food \& Drink & \grape \thinspace \wine \thinspace \fries & food-fruit, drink, food-vegetable \\
       Travel \& Places & \globe \thinspace \plane \thinspace \train & place-map, transportation-ground, transportation-air \\
       Activities & \wrestle \thinspace \biking \thinspace \ball & event, sport, game  \\
       Objects & \camera \thinspace \phone \thinspace \battery & sound, phone, money \\
       Symbol & \entry \thinspace \water \thinspace \rept & transport-sign, arrow, warning  \\
       Flags & \usa \thinspace \brazil \thinspace \iran & flag, country-flag \\
      \bottomrule
    \end{tabular}%
    }
\end{center}
\label{tab:emoji_order}
\end{table}


% \begin{figure}[ht]
% \centering
% \includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=0.75\textwidth]{figures/emj_category}
% \caption{Major orders of emoji}
% \label{fig:emoji_order}
% \end{figure}
















